Scabbard: An Exploratory Study on Hardware Aware Design Choices of Learning with Rounding-based Key Encapsulation Mechanisms

Recently, the construction of cryptographic schemes based on hard lattice problems has gained immense popularity. Apart from being quantum resistant, lattice-based cryptography allows a wide range of variations in the underlying hard problem. As cryptographic schemes can work in different environments under different operational constraints such as memory footprint, silicon area, efficiency, power requirement, etc., such variations in the underlying hard problem are very useful for designers to construct different cryptographic schemes. In this work, we explore various design choices of lattice-based cryptography and their impact on performance in the real world. In particular, we propose a suite of key-encapsulation mechanisms based on the learning with rounding problem with a focus on improving different performance aspects of lattice-based cryptography. Our suite consists of three schemes. Our first scheme is Florete, which is designed for efficiency. The second scheme is Espada, which is aimed at improving parallelization, flexibility, and memory footprint. The last scheme is Sable, which can be considered an improved version in terms of key sizes and parameters of the Saber key-encapsulation mechanism, one of the finalists in the National Institute of Standards and Technology's post-quantum standardization procedure. In this work, we have described our design rationale behind each scheme. Further, to demonstrate the justification of our design decisions, we have provided software and hardware implementations. Our results show Florete is faster than most state-of-the-art KEMs on software and hardware platforms. The scheme Espada requires less memory and area than the implementation of most state-of-the-art schemes. The implementations of Sable maintain a trade-off between Florete and Espada regarding performance and memory requirements on the hardware and software platform.

==> sections/hw_sw_implementation.tex <==
\section{HW/SW Co-Design} \label{sec:HWSWMULTIPLIER}
In order to demonstrate the design decisions of Scabbard, the polynomial multipliers are implemented in a HW/SW co-design. As a critical operation in lattice-based cryptography, including all Scabbard schemes, the polynomial multiplication is accelerated in hardware and all other operations are performed in software. However, as Scabbard was designed to be polynomial arithmetic-friendly, we use off the shelf and state-of-the-art polynomial multipliers in hardware. 

The following section discusses the particularities of our polynomial multiplier design for Florete, Espada and Sable. We demonstrate their efficiency, achieved through design decisions, in Section \ref{sec:resultHWSW}. In Section \ref{sec:HW_impl}, they are integrated in a full, high-performance hardware implementation.

\subsection{Florete}

\subsection{Espada}

\subsection{Sable}

\subsection{Results}\label{sec:resultHWSW}
We implement our HW-SW co-design on a Xilinx ZedBoard Zynq-7000 AP SoC device, which integrates an FPGA\footnote{XC7Z020-CLG484} and ARM Cortex-A9 processor. We use Vivado Design Suite 2018.1 and default strategies for synthesis and implementation.
Both processors communicate using an AXI interface and we use the DMA provided by Xilinx for a direct, streaming data transfer.


==> sections/parameters1.tex <==
\section{Parameter Set}\label{sec:parameters}

\textcolor{violet}{The lattice-based schemes whose hardness depends on the LWE problems or its variant, such as the (M/R)LWR problem, are solved by utilizing lattice reduction algorithms that construct a "sufficient orthogonal" basis from the given lattice. Currently the best-known algorithm for lattice reduction is the BKZ algorithm.} Here, given one lattice or a basis of lattice, the attacker needs to find the block size or sub-lattice size required for recovering the shortest vector of the lattice while performing the BKZ algorithm. The security of a lattice-based scheme depends on the cost of the execution time of the BKZ algorithm on the underlying lattice. The BKZ algorithm also calls the shortest vector problem (SVP) solving oracle on sub-lattices. The cost of solving the LWE problem with block size $\beta$ depends on the number of SVP oracle calls made by the BKZ algorithm and the cost of solving each SVP for dimension $\beta$. This cost is approximately $2^{c\beta+o(\beta)}$~\cite{LWE_estimator}, where the value of $c$ is approximately $0.292$ in classical settings and $0.265$ with Grover's speed-up algorithm~\cite{DBLP:conf/stoc/Grover96} in quantum settings.

\textcolor{violet}{Dachman-Soled et al.~\cite{leaky_estimator} has introduced leaky-LWE-Estimator, the state-of-the-art toolkit to estimate the hardness of the underlying LWE problem for lattice-based schemes.} This tool takes the $n=$ dimension of the lattice, $q=$ modulus, $D_e=$ error distribution, $D_s=$ secret distribution, and outputs the block size $\beta$. We have utilized this toolkit for the security estimation of our schemes. As the post-quantum security is lower than classical security $(0.292 > 0.265)$, we have mentioned only the post-quantum (PQ) security of our schemes in Table~\ref{table:parameters}. 

     

\begin{table}[!ht]
\centering
\scriptsize
\caption{Compare parameters and key sizes of Scabbard suite with Saber}
\label{table:parameters}
\begin{tabular}{lccccccccccc}
\hline
\multicolumn{1}{c}{{\color[HTML]{3531FF} \begin{tabular}[c]{@{}c@{}}\large{Scheme}\\ \large{Name}\end{tabular}}} & {\color[HTML]{3531FF} \begin{tabular}[c]{@{}c@{}}\large{Security}\\ \large{level}\end{tabular}} & \multicolumn{2}{c}{{\color[HTML]{3531FF} \begin{tabular}[c]{@{}c@{}}\large{Ring/Module}\\ \large{Parameters}\end{tabular}}} & {\color[HTML]{3531FF} \begin{tabular}[c]{@{}c@{}}\large{PQ}\\ \large{Security}\end{tabular}} & {\color[HTML]{3531FF} \begin{tabular}[c]{@{}c@{}}\large{Failure}\\ \large{probability}\end{tabular}} & \multicolumn{2}{c}{{\color[HTML]{3531FF} \large{Moduli}}} & {\color[HTML]{3531FF} \begin{tabular}[c]{@{}c@{}}\large{CBD}\\ \large{($\beta_\eta$)}\end{tabular}} & {\color[HTML]{3531FF} \large{Encoding}} & \multicolumn{2}{c}{{\color[HTML]{3531FF} \begin{tabular}[c]{@{}c@{}}\large{Key sizes for} \\ \large{KEM (Bytes)}\end{tabular}}} \\ \hline
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{512}                                                   & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_q$:}            & \large{11}             &                                                                                                     &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{608}                                     \\
                                                                                                                 & {\color[HTML]{FD6864} \large{Low}}                                                              &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{104}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-138}$}}                                                            & \large{$\epsilon_p$:}            & \large{9}              & \large{$\eta=1$}                                                                                    & \large{B=1}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{800}                                     \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{1}                                                     & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_t$:}            & \large{2}              &                                                                                                     &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{768}                                     \\ \cline{2-12} 
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{768}                                                   & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_q$:}            & \large{10}             &                                                                                                     &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{896}                                     \\
\multicolumn{1}{c}{{\color[HTML]{036400} \large{Florete}}}                                                       & {\color[HTML]{CB0000} \large{Medium}}                                                           &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{157}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-131}$}}                                                            & \large{$\epsilon_p$:}            & \large{9}              & \large{$\eta=1$}                                                                                    & \large{B=1}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{1152}                                    \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{1}                                                     & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_t$:}            & \large{3}              &                                                                                                     &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{1248}                                    \\ \cline{2-12} 
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{1024}                                                  & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_q$:}            & \large{10}             &                                                                                                     &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{1184}                                    \\
                                                                                                                 & {\color[HTML]{680100} \large{High}}                                                             &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{220}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-165}$}}                                                            & \large{$\epsilon_p$:}            & \large{9}              & \large{$\eta=1$}                                                                                    & \large{B=1}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{1504}                                    \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{1}                                                     & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_t$:}            & \large{4}              &                                                                                                     &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{1792}                                    \\ \hline
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{64}                                                    & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_q$:}            & \large{15}             &                                                                                                     &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{1072}                                    \\
                                                                                                                 & {\color[HTML]{FD6864} \large{Low}}                                                              &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{101}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-148}$}}                                                            & \large{$\epsilon_p$:}            & \large{13}             & \large{$\eta=3$}                                                                                    & \large{B=4}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{1456}                                    \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{10}                                                    & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_t$:}            & \large{2}              &                                                                                                     &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{1088}                                    \\ \cline{2-12} 
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{64}                                                    & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_q$:}            & \large{15}             &                                                                                                     &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{1280}                                    \\
\multicolumn{1}{c}{{\color[HTML]{036400} \large{Espada}}}                                                        & {\color[HTML]{CB0000} \large{Medium}}                                                           &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{128}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-167}$}}                                                            & \large{$\epsilon_p$:}            & \large{13}             & \large{$\eta=3$}                                                                                    & \large{B=4}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{1728}                                    \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{12}                                                    & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_t$:}            & \large{3}              &                                                                                                     &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{1304}                                    \\ \cline{2-12} 
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{64}                                                    & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_q$:}            & \large{15}             &                                                                                                     &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{1592}                                    \\
                                                                                                                 & {\color[HTML]{680100} \large{High}}                                                             &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{168}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-162}$}}                                                            & \large{$\epsilon_p$:}            & \large{13}             & \large{$\eta=3$}                                                                                    & \large{B=4}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{2136}                                    \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{15}                                                    & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_t$:}            & \large{5}              &                                                                                                     &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{1632}                                    \\ \hline
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{256}                                                   & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_q$:}            & \large{11}             &                                                                                                     &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{608}                                     \\
                                                                                                                 & {\color[HTML]{FD6864} \large{Low}}                                                              &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{104}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-139}$}}                                                            & \large{$\epsilon_p$:}            & \large{9}              & \large{$\eta=1$}                                                                                    & \large{B=1}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{800}                                     \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{2}                                                     & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_t$:}            & \large{2}              &                                                                                                     &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{672}                                     \\ \cline{2-12} 
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{256}                                                   & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_q$:}            & \large{11}             &                                                                                                     &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{896}                                     \\
\multicolumn{1}{c}{{\color[HTML]{036400} \large{Sable}}}                                                         & {\color[HTML]{CB0000} \large{Medium}}                                                           &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{169}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-143}$}}                                                            & \large{$\epsilon_p$:}            & \large{9}              & \large{$\eta=1$}                                                                                    & \large{B=1}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{1152}                                    \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{3}                                                     &                                                                                              & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_t$:}            & \large{4}              &                                                                                                     &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{1024}                                    \\ \cline{2-12} 
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{256}                                                   & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_q$:}            & \large{11}             &                                                                                                     &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{1312}                                    \\
                                                                                                                 & {\color[HTML]{680100} \large{High}}                                                             &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{203}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-208}$}}                                                            & \large{$\epsilon_p$:}            & \large{10}             & \large{$\eta=1$}                                                                                    & \large{B=1}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{1632}                                    \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{4}                                                     & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_t$:}            & \large{2}              &                                                                                                     &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{1376}                                    \\ \hline
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{256}                                                   & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_q$:}            & \large{13}             &                                                                                                     &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{672}                                     \\
                                                                                                                 & {\color[HTML]{FD6864} \large{Low}}                                                              &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{107}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-120}$}}                                                            & \large{$\epsilon_p$:}            & \large{10}             & \large{$\eta=5$}                                                                                    & \large{B=1}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{992}                                     \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{2}                                                     & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_t$:}            & \large{2}              &                                                                                                     &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{736}                                     \\ \cline{2-12} 
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{256}                                                   & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_q$:}            & \large{13}             &                                                                                                     &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{992}                                     \\
\multicolumn{1}{c}{{\color[HTML]{036400} \large{Saber}}}                                                         & {\color[HTML]{CB0000} \large{Medium}}                                                           &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{172}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-136}$}}                                                            & \large{$\epsilon_p$:}            & \large{10}             & \large{$\eta=4$}                                                                                    & \large{B=1}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{1440}                                    \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{3}                                                     & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_t$:}            & \large{3}              &                                                                                                     &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{1088}                                    \\ \cline{2-12} 
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{256}                                                   & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_q$:}            & \large{13}             &                                                                                                     &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{1312}                                    \\
                                                                                                                 & {\color[HTML]{680100} \large{High}}                                                             &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{236}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-165}$}}                                                            & \large{$\epsilon_p$:}            & \large{10}             & \large{$\eta=3$}                                                                                    & \large{B=1}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{1760}                                    \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{4}                                                     &                                                                                              &                                                                                                      & \large{$\epsilon_t$:}            & \large{5}              &                                                                                                     &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{1472}                                    \\ \hline
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{256}                                                   & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$q$:}                     & \large{3329}           & \large{$\eta_1=3$}                                                                                  &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{800}                                     \\
                                                                                                                 & {\color[HTML]{FD6864} \large{Low}}                                                              &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{107}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-139}$}}                                                            & \large{$\epsilon_p$:}            & \large{10}             &                                                                                                     & \large{B=1}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{1632}                                    \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{2}                                                     & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_t$:}            & \large{3}              & \large{$\eta_2=2$}                                                                                  &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{768}                                     \\ \cline{2-12} 
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{256}                                                   & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$q$:}                     & \large{3329}           & \large{$\eta_1=2$}                                                                                  &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{1184}                                    \\
\multicolumn{1}{c}{{\color[HTML]{036400} \large{Kyber}}}                                                         & {\color[HTML]{CB0000} \large{Medium}}                                                           &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{166}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-164}$}}                                                            & \large{$\epsilon_p$:}            & \large{10}             &                                                                                                     & \large{B=1}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{2400}                                    \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{3}                                                     & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$\epsilon_t$:}            & \large{3}              & \large{$\eta_2=2$}                                                                                  &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{1088}                                    \\ \cline{2-12} 
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{n:}                                                  & \large{256}                                                   & {\color[HTML]{CB0000} }                                                                      & {\color[HTML]{CB0000} }                                                                              & \large{$q$:}                     & \large{3329}           & \large{$\eta_1=2$}                                                                                  &                                         & {\color[HTML]{036400} \large{Public key:}}                                    & \large{1568}                                    \\
                                                                                                                 & {\color[HTML]{680100} \large{High}}                                                             &                                                             &                                                               & {\color[HTML]{CB0000} \large{$2^{232}$}}                                                     & {\color[HTML]{CB0000} \large{$2^{-174}$}}                                                            & \large{$\epsilon_p$:}            & \large{10}             &                                                                                                     & \large{B=1}                             & {\color[HTML]{036400} \large{Secret key:}}                                    & \large{3168}                                    \\
                                                                                                                 & {\color[HTML]{036400} }                                                                         & \large{l:}                                                  & \large{4}                                                     &                                                                                              &                                                                                                      & \large{$\epsilon_t$:}            & \large{4}              & \large{$\eta_2=2$}                                                                                  &                                         & {\color[HTML]{036400} \large{Ciphertext:}}                                    & \large{1568}                                    \\ \hline
\end{tabular}
\end{table}

\textcolor{violet}{We present the parameter sets of our schemes for three security levels in Table~\ref{table:parameters}}. For security level $1$, PQ security of each of the KEMs is $\geq 2^{100}$, for security level $3$, PQ security is $\geq 2^{128}$, and for security level $5$, PQ security is $\geq 2^{160}$. 
LWE-based cryptosystem has another security factor which is failure probability. 
\textcolor{violet}{However, another type of attack is possible on LWR or LWR-based cryptographic schemes that exploit failure probability during decryption.}
As mentioned in Sec.~\ref{sec:genericLWR}, the failure probability should be $\leq 2^{-S}$, where $S$ is the security of the KEM to maintain the IND-CCA security of the KEM. Therefore, for security level $1, 3, 5$ in contrast with the PQ security, the failure probability we maintain $\leq 2^{-100}, \leq 2^{-128}, \leq 2^{-160}$, respectively for each of the KEMs. NIST security levels $1$, $3$, and $5$ are represented by low, medium, and high-security levels in Table~\ref{table:parameters}.  

For comparing the key sizes of our schemes with Saber and Kyber, we also include the parameter sets of Saber in Table~\ref{table:parameters}. The public key and secret key sizes of Florete are smaller than Saber, while the size of the ciphertext is slightly larger for Florete than Saber for all three security levels. The public key and secret key sizes of Florete are also smaller than Kyber for all three security versions. Even, the size of the ciphertext is the same for the low-security version of Florete and Kyber. Due to larger moduli and vector dimensions, the public key, secret key, and ciphertext sizes are bigger in Espada than in Saber for the same security level. However, the secret key size of Espada is smaller in Espada than in Kyber for all the security versions. In the case of any of the three security levels of Sable, the sizes of the public key, secret key, and ciphertext are smaller than in the case of the same security level of Saber and Kyber. 
























% \begin{table}[t]
% \centering
% \caption{Compare parameters and key sizes of Scabbard suite with Saber}
% \label{table:parameters}
% \begin{tabular}{lccccccccccc}
% \hline
% \multicolumn{1}{c}{{\color[HTML]{3531FF} Scheme}} & {\color[HTML]{3531FF} Security level} & \multicolumn{2}{c}{{\color[HTML]{3531FF} \begin{tabular}[c]{@{}c@{}}Ring/Module\\ Parameters\end{tabular}}} & {\color[HTML]{3531FF} \begin{tabular}[c]{@{}c@{}}PQ\\ Security\end{tabular}} & {\color[HTML]{3531FF} \begin{tabular}[c]{@{}c@{}}Failure\\ probability\end{tabular}} & \multicolumn{2}{c}{{\color[HTML]{3531FF} Moduli}} & {\color[HTML]{3531FF} \begin{tabular}[c]{@{}c@{}}CBD\\ ($\beta_\mu$)\end{tabular}} & {\color[HTML]{3531FF} Encoding} & \multicolumn{2}{c}{{\color[HTML]{3531FF} \begin{tabular}[c]{@{}c@{}}Key sizes for \\ KEM (Bytes)\end{tabular}}} \\ \hline
%                                                        & {\color[HTML]{036400} }               & {n:}                                                & {512}                                                 & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_q$:}               & {11}              &                                                                                     &                                 & {\color[HTML]{036400} {Public key:}}                                  & {608}                                   \\
%                                                        & {\color[HTML]{FD6864} {Low}}            &                                                     &                                                       & {\color[HTML]{CB0000} {$2^{104}$}}                                           & {\color[HTML]{CB0000} {$2^{-138}$}}                                                  & {$\epsilon_p$:}               & {9}               & {$\mu=1$}                                                                          & {B=1}                           & {\color[HTML]{036400} {Secret key:}}                                  & {800}                                   \\
%                                                        & {\color[HTML]{036400} }               & {l:}                                                & {1}                                                   & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_t$:}               & {2}               &                                                                                     &                                 & {\color[HTML]{036400} {Ciphertext:}}                                  & {768}                                   \\ \cline{2-12} 
%                                                        & {\color[HTML]{036400} }               & {n:}                                                & {768}                                                 & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_q$:}               & {10}              &                                                                                     &                                 & {\color[HTML]{036400} {Public key:}}                                  & {896}                                   \\
% \multicolumn{1}{c}{{\color[HTML]{036400} {Florete}}}   & {\color[HTML]{CB0000} {Medium}}            &                                                     &                                                       & {\color[HTML]{CB0000} {$2^{157}$}}                                           & {\color[HTML]{CB0000} {$2^{-131}$}}                                                  & {$\epsilon_p$:}               & {9}               & {$\mu=1$}                                                                          & {B=1}                           & {\color[HTML]{036400} {Secret key:}}                                  & {1152}                                  \\
%                                                        & {\color[HTML]{036400} }               & {l:}                                                & {1}                                                   & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_t$:}               & {3}               &                                                                                     &                                 & {\color[HTML]{036400} {Ciphertext:}}                                  & {1248}                                  \\ \cline{2-12} 
%                                                        & {\color[HTML]{036400} }               & {n:}                                                & {1024}                                                & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_q$:}               & {10}              &                                                                                     &                                 & {\color[HTML]{036400} {Public key:}}                                  & {1184}                                  \\
%                                                        & {\color[HTML]{680100} {High}}            &                                                     &                                                       & {\color[HTML]{CB0000} {$2^{220}$}}                                           & {\color[HTML]{CB0000} {$2^{-165}$}}                                                  & {$\epsilon_p$:}               & {9}               & {$\mu=1$}                                                                          & {B=1}                           & {\color[HTML]{036400} {Secret key:}}                                  & {1504}                                  \\
%                                                        & {\color[HTML]{036400} }               & {l:}                                                & {1}                                                   & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_t$:}               & {4}               &                                                                                     &                                 & {\color[HTML]{036400} {Ciphertext:}}                                  & {1792}                                  \\ \hline
%                                                        & {\color[HTML]{036400} }               & {n:}                                                & {64}                                                  & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_q$:}               & {15}              &                                                                                     &                                 & {\color[HTML]{036400} {Public key:}}                                  & {1072}                                  \\
%                                                        & {\color[HTML]{FD6864} {Low}}            &                                                     &                                                       & {\color[HTML]{CB0000} {$2^{101}$}}                                           & {\color[HTML]{CB0000} {$2^{-148}$}}                                                  & {$\epsilon_p$:}               & {13}              & {$\mu=3$}                                                                          & {B=4}                           & {\color[HTML]{036400} {Secret key:}}                                  & {1456}                                  \\
%                                                        & {\color[HTML]{036400} }               & {l:}                                                & {10}                                                  & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_t$:}               & {2}               &                                                                                     &                                 & {\color[HTML]{036400} {Ciphertext:}}                                  & {1088}                                  \\ \cline{2-12} 
%                                                        & {\color[HTML]{036400} }               & {n:}                                                & {64}                                                  & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_q$:}               & {15}              &                                                                                     &                                 & {\color[HTML]{036400} {Public key:}}                                  & {1280}                                  \\
% \multicolumn{1}{c}{{\color[HTML]{036400} {Espada}}}    & {\color[HTML]{CB0000} {Medium}}            &                                                     &                                                       & {\color[HTML]{CB0000} {$2^{128}$}}                                           & {\color[HTML]{CB0000} {$2^{-167}$}}                                                  & {$\epsilon_p$:}               & {13}              & {$\mu=3$}                                                                          & {B=4}                           & {\color[HTML]{036400} {Secret key:}}                                  & {1728}                                  \\
%                                                        & {\color[HTML]{036400} }               & {l:}                                                & {12}                                                  & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_t$:}               & {3}               &                                                                                     &                                 & {\color[HTML]{036400} {Ciphertext:}}                                  & {1304}                                  \\ \cline{2-12} 
%                                                        & {\color[HTML]{036400} }               & {n:}                                                & {64}                                                  & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_q$:}               & {15}              &                                                                                     &                                 & {\color[HTML]{036400} {Public key:}}                                  & {1592}                                  \\
%                                                        & {\color[HTML]{680100} {High}}            &                                                     &                                                       & {\color[HTML]{CB0000} {$2^{168}$}}                                           & {\color[HTML]{CB0000} {$2^{-162}$}}                                                  & {$\epsilon_p$:}               & {13}              & {$\mu=3$}                                                                          & {B=4}                           & {\color[HTML]{036400} {Secret key:}}                                  & {2136}                                  \\
%                                                        & {\color[HTML]{036400} }               & {l:}                                                & {15}                                                  & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_t$:}               & {5}               &                                                                                     &                                 & {\color[HTML]{036400} {Ciphertext:}}                                  & {1632}                                  \\ \hline
%                                                        & {\color[HTML]{036400} }               & {n:}                                                & {256}                                                 & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_q$:}               & {11}              &                                                                                     &                                 & {\color[HTML]{036400} {Public key:}}                                  & {608}                                   \\
%                                                        & {\color[HTML]{FD6864} {Low}}            &                                                     &                                                       & {\color[HTML]{CB0000} {$2^{104}$}}                                           & {\color[HTML]{CB0000} {$2^{-139}$}}                                                  & {$\epsilon_p$:}               & {9}               & {$\mu=1$}                                                                          & {B=1}                           & {\color[HTML]{036400} {Secret key:}}                                  & {800}                                   \\
%                                                        & {\color[HTML]{036400} }               & {l:}                                                & {2}                                                   & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_t$:}               & {2}               &                                                                                     &                                 & {\color[HTML]{036400} {Ciphertext:}}                                  & {672}                                   \\ \cline{2-12} 
%                                                        & {\color[HTML]{036400} }               & {n:}                                                & {256}                                                 & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_q$:}               & {11}              &                                                                                     &                                 & {\color[HTML]{036400} {Public key:}}                                  & {896}                                   \\
% \multicolumn{1}{c}{{\color[HTML]{036400} {Sable}}}     & {\color[HTML]{CB0000} {Medium}}            &                                                     &                                                       & {\color[HTML]{CB0000} {$2^{169}$}}                                           & {\color[HTML]{CB0000} {$2^{-143}$}}                                                  & {$\epsilon_p$:}               & {9}               & {$\mu=1$}                                                                          & {B=1}                           & {\color[HTML]{036400} {Secret key:}}                                  & {1152}                                  \\
%                                                        & {\color[HTML]{036400} }               & {l:}                                                & {3}                                                   &                                                                              & {\color[HTML]{CB0000} }                                                              & {$\epsilon_t$:}               & {4}               &                                                                                     &                                 & {\color[HTML]{036400} {Ciphertext:}}                                  & {1024}                                  \\ \cline{2-12} 
%                                                        & {\color[HTML]{036400} }               & {n:}                                                & {256}                                                 & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_q$:}               & {11}              &                                                                                     &                                 & {\color[HTML]{036400} {Public key:}}                                  & {1312}                                  \\
%                                                        & {\color[HTML]{680100} {High}}            &                                                     &                                                       & {\color[HTML]{CB0000} {$2^{203}$}}                                           & {\color[HTML]{CB0000} {$2^{-208}$}}                                                  & {$\epsilon_p$:}               & {10}              & {$\mu=1$}                                                                          & {B=1}                           & {\color[HTML]{036400} {Secret key:}}                                  & {1632}                                  \\
%                                                        & {\color[HTML]{036400} }               & {l:}                                                & {4}                                                   & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_t$:}               & {2}               &                                                                                     &                                 & {\color[HTML]{036400} {Ciphertext:}}                                  & {1376}                                  \\ \hline
%                                                        & {\color[HTML]{036400} }               & {n:}                                                & {256}                                                 & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_q$:}               & {13}              &                                                                                     &                                 & {\color[HTML]{036400} {Public key:}}                                  & {672}                                   \\
%                                                        & {\color[HTML]{FD6864} {Low}}            &                                                     &                                                       & {\color[HTML]{CB0000} {$2^{107}$}}                                           & {\color[HTML]{CB0000} {$2^{-120}$}}                                                  & {$\epsilon_p$:}               & {10}              & {$\mu=5$}                                                                          & {B=1}                           & {\color[HTML]{036400} {Secret key:}}                                  & {992}                                   \\
%                                                        & {\color[HTML]{036400} }               & {l:}                                                & {2}                                                   & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_t$:}               & {2}               &                                                                                     &                                 & {\color[HTML]{036400} {Ciphertext:}}                                  & {736}                                   \\ \cline{2-12} 
%                                                        & {\color[HTML]{036400} }               & {n:}                                                & {256}                                                 & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_q$:}               & {13}              &                                                                                     &                                 & {\color[HTML]{036400} {Public key:}}                                  & {992}                                   \\
% \multicolumn{1}{c}{{\color[HTML]{036400} {Saber}}}     & {\color[HTML]{CB0000} {Medium}}            &                                                     &                                                       & {\color[HTML]{CB0000} {$2^{172}$}}                                           & {\color[HTML]{CB0000} {$2^{-136}$}}                                                  & {$\epsilon_p$:}               & {10}              & {$\mu=4$}                                                                          & {B=1}                           & {\color[HTML]{036400} {Secret key:}}                                  & {1440}                                  \\
%                                                        & {\color[HTML]{036400} }               & {l:}                                                & {3}                                                   & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_t$:}               & {3}               &                                                                                     &                                 & {\color[HTML]{036400} {Ciphertext:}}                                  & {1088}                                  \\ \cline{2-12} 
%                                                        & {\color[HTML]{036400} }               & {n:}                                                & {256}                                                 & {\color[HTML]{CB0000} }                                                      & {\color[HTML]{CB0000} }                                                              & {$\epsilon_q$:}               & {13}              &                                                                                     &                                 & {\color[HTML]{036400} {Public key:}}                                  & {1312}                                  \\
%                                                        & {\color[HTML]{680100} {High}}            &                                                     &                                                       & {\color[HTML]{CB0000} {$2^{236}$}}                                           & {\color[HTML]{CB0000} {$2^{-165}$}}                                                  & {$\epsilon_p$:}               & {10}              & {$\mu=3$}                                                                          & {B=1}                           & {\color[HTML]{036400} {Secret key:}}                                  & {1760}                                  \\
%                                                        & {\color[HTML]{036400} }               & {l:}                                                & {4}                                                   &                                                                              &                                                                                      & {$\epsilon_t$:}               & {5}               &                                                                                     &                                 & {\color[HTML]{036400} {Ciphertext:}}                                  & {1472}                                  \\ \hline
% \end{tabular}
% \end{table}


% --------------------OLD-----------------------------------
